Open Source Language Models Can Provide Feedback: Evaluating LLMs' Ability to Help Students Using GPT-4-As-A-Judge

Large language models (LLMs) have shown great potential for the automatic generation of feedback in a wide range of computing contexts. However, concerns have been voiced around the privacy and ethical implications of sending student work to proprietary models. This has sparked considerable interest in the use of open source LLMs in education, but the quality of the feedback that such open models can produce remains understudied. This is a concern as providing flawed or misleading generated feedback could be detrimental to student learning. Inspired by recent work that has utilised very powerful LLMs, such as GPT-4, to evaluate the outputs produced by less powerful models, we conduct an automated analysis of the quality of the feedback produced by several open source models using a dataset from an introductory programming course. First, we investigate the viability of employing GPT-4 as an automated evaluator by comparing its evaluations with those of a human expert. We observe that GPT-4 demonstrates a bias toward positively rating feedback while exhibiting moderate agreement with human raters, showcasing its potential as a feedback evaluator. Second, we explore the quality of feedback generated by several leading open-source LLMs by using GPT-4 to evaluate the feedback. We find that some models offer competitive performance with popular proprietary LLMs, such as ChatGPT, indicating opportunities for their responsible use in educational settings.

==> data/figure/benchmark_figure.tex <==
\begin{figure}[htbp]
    \centering

    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth,trim={2.7cm 0 0 0},clip]{images/codellama_34b_upsetplot_subset.pdf}
        \caption{CodeLLAMA 34b results}
        \label{fig:subfig4}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth,trim={2.7cm 0 0 0},clip]{images/zephyr_beta_7b_upsetplot_subset.pdf}
        \caption{Zephyr 7B results}
        \label{fig:subfig1}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth,trim={2.7cm 0 0 0},clip]
        {images/gpt-3.5-turbo_upsetplot_subset.pdf}
        \caption{GPT3.5 results}
        \label{fig:subfig5}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth,trim={2.7cm 0 0 0},clip]
        {images/gpt-4_upsetplot_subset.pdf}
        \caption{GPT-4 results}
        \label{fig:subfig6}
    \end{subfigure}

    % explanations 
    \begin{tikzpicture}[overlay, remember picture]
        \node at (current page.center) [anchor=center, yshift=11.15cm,xshift=-6.5cm]
            {\boldcircled{1}};
    \end{tikzpicture}

    \caption{Feedback quality results for different language models. These Upset plots depict the count of feedback meeting intersections of specific criteria. Legend -  Full-blue: insightful, Full-orange: comprehensive feedback.}

    \label{fig:feedback_results}
\end{figure}

\endinput 

% 
\begin{tikzpicture}[overlay, remember picture]
    \node at (current page.center) [anchor=center, yshift=7.3cm,xshift=-7.2cm]
        {\boldcircled{2}};
\end{tikzpicture}



\todo[inline]{crop the bars on the left to get more space, and get 4 on one line.}

\todo[inline]{One of the bars should be full there}

==> data/figure/benchmark_figure_subset.tex <==
\begin{figure*}[htbp]
    \centering

    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth,trim={2.7cm 0 0 0},clip]{images/codellama_34b_upsetplot_subset.pdf}
        \caption{CodeLLAMA 34b results}
        \label{fig:subfig4}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth,trim={2.7cm 0 0 0},clip]{images/zephyr_beta_7b_upsetplot_subset.pdf}
        \caption{Zephyr 7B results}
        \label{fig:subfig1}
    \end{subfigure}%
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth,trim={2.7cm 0 0 0},clip]
        {images/gpt-3.5-turbo_upsetplot_subset.pdf}
        \caption{GPT3.5 results}
        \label{fig:subfig5}
    \end{subfigure}%
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth,trim={2.7cm 0 0 0},clip]
        {images/gpt-4_upsetplot_subset.pdf}
        \caption{GPT-4 results}
        \label{fig:subfig6}
    \end{subfigure}

    \caption{Feedback quality results for different language models. These Upset plots depict the count of feedback meeting intersections of specific criteria. Legend -  Full-blue: insightful, Full-orange: comprehensive feedback.}

    \label{fig:feedback_results}
\end{figure*}

\endinput 

% explanations 
\begin{tikzpicture}[overlay, remember picture]
    \node at (current page.center) [anchor=center, yshift=11.15cm,xshift=-6.5cm]
        {\boldcircled{1}};
\end{tikzpicture}
% 
\begin{tikzpicture}[overlay, remember picture]
    \node at (current page.center) [anchor=center, yshift=7.3cm,xshift=-7.2cm]
        {\boldcircled{2}};
\end{tikzpicture}



\todo[inline]{crop the bars on the left to get more space, and get 4 on one line.}

\todo[inline]{One of the bars should be full there}

==> data/figure/ground_truth_upset_plot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth,trim={2.50cm 0.75cm 0 0},clip]{images/ground_truth_upsetplot.pdf}
    \caption{Ground truth upset plot.}
    \label{fig:gt_upset}
\end{figure}

==> data/prompts/grading_prompt.tex <==
\begin{figure}[htbp!]
\centering
\begin{example}{Prompting GPT-4 to grade LLM generated feedback}
You are a computer science professor 
teaching introductory programming using Dart. \circled{1} \\ 

Below is a problem description, a model solution, and an incorrect program written by a student. You are also provided with the feedback on the generated by GPT3.5. Your task is to evaluate the quality of the feedback (by saying yes or no) to ensure it adheres to the multiple criteria outlined below. For each criterion, provide your answer in a separate line with the format \textquotesingle (CRITERIA\_NUMBER): Yes/No\textquotesingle. Do not provide comments, but be attentive to the problem description requirements. \circled{2} \\ 
\vspace{-0.1cm}
\hspace{7.23cm} \tikzmark{startBracket} \\
\vspace{-0.1cm}
\#\# Problem description: \\ 

\textcolor{blue}{<handout>} \\ 

\#\#  Model solution: \\ 

\textcolor{blue}{<sample\_solution>} \\ 

\#\#  Student Code: \\ 

\textcolor{blue}{<submitted\_code>} \\

\#\#  Feedback: \\ 

\textcolor{blue}{<feedback>} \\ 

\#\#  Criteria: \\ 

(1) Identifies and mentions all actual issues \\ 
(2) Identifies and mentions at least one actual issue \\ 
(3) Does not identify non-existent issues \\ 
(4) Does not produce unnecessary, duplicate, or repetitive content \\ 

\vspace{-0.5cm} \hspace{7.33cm} \tikzmark{endBracket}  

\#\#  Answer: \\ 
\vspace{-0.4cm}
\hspace{4.3cm} \tikzmark{startBracket2} \\

(1): \textcolor{blue}{True/False} \\ 
(2): \textcolor{blue}{True/False} \\ 
(3): \textcolor{blue}{True/False} \\ 
(4): \textcolor{blue}{True/False} \\

\#\# Problem description: \textcolor{blue}{<new\_handout>} \\ 
\Large{\textbf{...}} \\
\vspace{-0.5cm} \hspace{4.3cm} \tikzmark{endBracket2}

% Draw brackets using tikz
\begin{tikzpicture}[overlay, remember picture]
  \draw[decorate, decoration={brace, amplitude=7pt, raise=4pt}] (pic cs:startBracket) -- (pic cs:endBracket) node[midway, right=0.32cm] {\smallcircled{3}};
  \draw[decorate, decoration={brace, amplitude=10pt, raise=4pt}] (pic cs:startBracket2) -- (pic cs:endBracket2) node[midway, right=0.4cm] {\smallcircled{4}};
\end{tikzpicture}

\end{example}
\caption{Our template for prompting the LLMs to provide feedback. (1) A system prompt specifying the behaviour of the model. (2) A description of the grading task. (3) Information necessary to grade the feedback. When zero-shot prompting, the prompt stops there; when one-shot prompting, we provide (4) the ground truth annotation answer for the given submitted code and feedback before we format once more the information for the feedback being graded.}
\label{fig:grading_prompt}
\end{figure}

==> data/table/feedback_separate.tex <==
\begin{table}[htbp]
\caption{Separate model results}
\label{tab:feed_res}
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|ccccc}
\toprule
model & size & completeness & concision & perceptivity & selectivity \\
\midrule
zephyr\_beta & 7b & 0.86 & 0.76 & 0.97 & 0.79 \\
gpt-3.5-turbo & / & 0.89 & 0.90 & 0.99 & 0.77 \\
codellama & 7b & 0.62 & 0.57 & 0.99 & 0.27 \\
codellama & 34b & 0.77 & 0.78 & 0.99 & 0.49 \\
codellama & 13b & 0.73 & 0.77 & 0.95 & 0.63 \\
\bottomrule
\end{tabular}
}
\end{table}


==> data/table/grading_4_rows/grading_all.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & \textbf{f0.5} & f1 & accuracy & kappa \\
\midrule
0S & 0.80 & 0.97 & \textbf{0.83} & 0.88 & 0.81 & 0.43 \\
1S-O & 0.81 & 0.97 & \textbf{0.83} & 0.88 & 0.81 & 0.45 \\
1S-S & 0.83 & 0.96 & \textbf{0.85} & 0.89 & 0.83 & 0.53 \\
\bottomrule
\end{tabular}

==> data/table/grading_4_rows/grading_completeness.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & \textbf{f0.5} & f1 & accuracy & kappa \\
\midrule
0S & 0.69 & 0.98 & \textbf{0.73} & 0.81 & 0.75 & 0.47 \\
1S-O & 0.69 & 0.91 & \textbf{0.73} & 0.79 & 0.73 & 0.44 \\
1S-S & 0.74 & 0.87 & \textbf{0.76} & 0.80 & 0.76 & 0.51 \\
\bottomrule
\end{tabular}

==> data/table/grading_4_rows/grading_concision.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & \textbf{f0.5} & f1 & accuracy & kappa \\
\midrule
0S & 0.98 & 0.98 & \textbf{0.98} & 0.98 & 0.96 & -0.02 \\
1S-O & 0.98 & 0.99 & \textbf{0.98} & 0.99 & 0.97 & -0.01 \\
1S-S & 0.98 & 1.00 & \textbf{0.98} & 0.99 & 0.98 & 0.00 \\
\bottomrule
\end{tabular}

==> data/table/grading_4_rows/grading_perceptivity.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & \textbf{f0.5} & f1 & accuracy & kappa \\
\midrule
0S & 0.85 & 0.98 & \textbf{0.87} & 0.91 & 0.84 & 0.27 \\
1S-O & 0.87 & 0.96 & \textbf{0.88} & 0.91 & 0.85 & 0.36 \\
1S-S & 0.87 & 0.95 & \textbf{0.89} & 0.91 & 0.85 & 0.38 \\
\bottomrule
\end{tabular}

==> data/table/grading_4_rows/grading_selectivity.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & \textbf{f0.5} & f1 & accuracy & kappa \\
\midrule
0S & 0.62 & 0.96 & \textbf{0.67} & 0.76 & 0.68 & 0.34 \\
1S-O & 0.63 & 0.97 & \textbf{0.68} & 0.76 & 0.69 & 0.36 \\
1S-S & 0.66 & 0.99 & \textbf{0.71} & 0.79 & 0.73 & 0.45 \\
\bottomrule
\end{tabular}

==> data/table/grading_4_rows/overall_stats.tex <==
\begin{tabular}{r|cc}
\toprule
 & False & True \\
\midrule
completeness & 68 & 82 \\
perceptivity & 27 & 123 \\
selectivity & 72 & 78 \\
concision & 3 & 147 \\
\bottomrule
\end{tabular}

==> data/table/grading_4_rows/table.tex <==
\begin{table}[hbtp]
\small
\caption{Ground truth grading criteria statistics. Number of generated feedback classified under each criteria.}

\label{tab: grad_stat}
\begin{tabular}{r|cc}
\toprule
 & False & True \\
\midrule
completeness & 68 & 82 \\
perceptivity & 27 & 123 \\
selectivity & 72 & 78 \\
concision & 3 & 147 \\
\bottomrule
\end{tabular}

\vspace{0.5cm}

\caption{GPT-4 Grading results. The first table shows the average of the scores for all criteria, and the four following tables detail the scores for each individual criterion. Legend: (0S) zero-shot, (1S-O) one-shot using feedback for another assignment, (1S-S) one-shot using feedback for another help request for the same assignment.}

\label{tab: grading_results}
\begin{subcaptiongroup}

\begin{minipage}{\columnwidth}
\caption{all: completeness, perceptivity, selectivity, concision}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_4_rows/grading_all}
}
\end{minipage}%

\vspace{0.5cm}
%\noindent\rule{9cm}{0.4pt}

\begin{minipage}{\columnwidth}
\caption{completness}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_4_rows/grading_completeness}
}
\end{minipage}%

\vspace{0.1cm}

\begin{minipage}{\columnwidth}
\caption{perceptivity}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_4_rows/grading_perceptivity}
}
\end{minipage}%

\vspace{0.1cm}

\begin{minipage}{\columnwidth}
\caption{selectivity}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_4_rows/grading_selectivity}
}
\end{minipage}%

\vspace{0.1cm}

\begin{minipage}{\columnwidth}
\caption{concision}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_4_rows/grading_concision}
}
\end{minipage}%

\end{subcaptiongroup}
\end{table}


==> data/table/grading_criteria_together/dummy_scores.tex <==
\begin{tabular}{lcc|c|ccc}
\toprule
 & precision & recall & f0.5 & f1 & accuracy & kappa \\
\midrule
completeness & 0.55 & 1.00 & 0.60 & 0.71 & 0.55 & 0.00 \\
perceptivity & 0.82 & 1.00 & 0.85 & 0.90 & 0.82 & 0.00 \\
selectivity & 0.52 & 1.00 & 0.58 & 0.68 & 0.52 & 0.00 \\
concision & 0.98 & 1.00 & 0.98 & 0.99 & 0.98 & 0.00 \\
\hline
all & 0.72 & 1.00 & 0.76 & 0.83 & 0.72 & 0.00 \\
\bottomrule
\end{tabular}


==> data/table/grading_criteria_together/full_table.tex <==
\begin{table}[hbtp]
\small

\caption{Ground truth grading criteria statistics. Number of generated feedback classified under each criteria.}

\label{tab: grad_stat}
\begin{tabular}{r|cc}
\toprule
 & False & True \\
\midrule
completeness & 68 & 82 \\
perceptivity & 27 & 123 \\
selectivity & 72 & 78 \\
concision & 3 & 147 \\
\bottomrule
\end{tabular}

\vspace{0.5cm}

\caption{GPT-4 Grading results. The first table shows the average of the scores for all criteria, and the four following tables detail the scores for each individual criterion. Legend: (0S) zero-shot, (1S-O) one-shot using feedback for another assignment, (1S-S) one-shot using feedback for another help request for the same assignment.}

\label{tab: grading_results}
\begin{subcaptiongroup}

\begin{minipage}{\columnwidth}
\caption{zero-shot grading}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_criteria_together/zero_shot}
}
\end{minipage}%

\vspace{0.5cm}
%\noindent\rule{9cm}{0.4pt}

\begin{minipage}{\columnwidth}
\caption{completness}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_criteria_together/one_shot_other}
}
\end{minipage}%

\vspace{0.1cm}

\begin{minipage}{\columnwidth}
\caption{perceptivity}
\resizebox{\linewidth}{!}{%
\input{data/table/grading_criteria_together/one_shot_same}
}
\end{minipage}%

\end{subcaptiongroup}
\end{table}


==> data/table/grading_criteria_together/one_shot_other.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & f0.5 & f1 & accuracy & kappa \\
\midrule
completeness & 0.70 & 0.95 & 0.74 & 0.81 & 0.75 & 0.48 \\
perceptivity & 0.86 & 0.96 & 0.88 & 0.91 & 0.84 & 0.32 \\
selectivity & 0.58 & 1.00 & 0.64 & 0.74 & 0.63 & 0.23 \\
concision & 0.98 & 0.99 & 0.98 & 0.99 & 0.97 & -0.01 \\\midrule 
all & 0.79 & 0.98 & \textbf{0.82} & 0.87 & 0.80 & 0.39 \\
\bottomrule
\end{tabular}

==> data/table/grading_criteria_together/one_shot_same.tex <==
\begin{tabular}{r|cc|c|ccc}
\small
\toprule
 & precision & recall & f0.5 & f1 & accuracy & kappa \\
\midrule
completeness & 0.71 & 0.94 & 0.74 & 0.81 & 0.75 & 0.48 \\
perceptivity & 0.88 & 0.96 & 0.90 & 0.92 & 0.86 & 0.44 \\
selectivity & 0.60 & 0.96 & 0.64 & 0.74 & 0.64 & 0.26 \\
concision & 0.98 & 0.99 & 0.98 & 0.99 & 0.97 & -0.01 \\\midrule 
all & 0.80 & 0.97 & \textbf{0.83} & 0.88 & 0.81 & 0.44 \\
\bottomrule
\end{tabular}


==> sections/eval_feedback.tex <==
\section{Large Language Models can Evaluate Feedback Quality}
% Using GPT-4 as an evaluator 
Prior work suggests that GPT-4 can act as a good evaluator. To confirm that scenario in our setup, we conduct a small study on our data to test the extent to which GPT-4 agrees with human evaluators.

We use the data from the study \cite{hellas2023exploring}. We compare the results in detail in terms of "identifies all issues", "identifies at least one issue", etc. 

\todo[inline]{Need Arto's data}
Small-scale evaluation of which is preferred by educators 

Our results suggest that, in particular for research, we can rely on GPT-4 for comparing the accuracy of feedback methods. We propose to look at benchmarking datasets (open-source) and for them to use GPT-4 to look at the quality of feedback or when we can provide this feedback. 


\section{Benchmarking Language Models for Programming Feedback}

We have established that GPT-4 can be used as a reliable feedback quality evaluator in specific cases. We now use our discovery to scale the automated evaluation of programming feedback on several benchmarks. 

We then take a look at the quality of feedback given by various language models using GPT-4 as our evaluator. How do permissive models compare against their non-permissive counterparts? 

We define feedback as "accurate" if it addresses all the issues in the student solution. We

We note the following: although a model would not always be good at identifying all issues, perhaps the model could be good at identifying one issue, which could be provided as a single-step hint to students. We evaluate this scenario, by recursively asking a single model to identify one issue in the program and looking at whether eventually all the issues have been successfully identified. 

---------

We conduct our evaluation focusing on Python and javascript code and leave the rest for future work 




\todo[inline]{Quality also using the other "identify one issue, etc."}





\endinput 

